Relation Embedding for Personalised POI Recommendation

Point-of-Interest (POI) recommendation is one of the most important location-based services helping people discover interesting venues or services. However, the extreme user-POI matrix sparsity and the varying spatio-temporal context pose challenges for POI systems, which affects the quality of POI recommendations. To this end, we propose a translation-based relation embedding for POI recommendation. Our approach encodes the temporal and geographic information, as well as semantic contents effectively in a low-dimensional relation space by using Knowledge Graph Embedding techniques. To further alleviate the issue of user-POI matrix sparsity, a combined matrix factorization framework is built on a user-POI graph to enhance the inference of dynamic personal interests by exploiting the side-information. Experiments on two real-world datasets demonstrate the effectiveness of our proposed model.

==> sections/preliminaries.tex <==
\section{Problem Definition}
Notations which are frequently used in the remainder of this paper are summarized in Table \ref{tb:notations}. 


\begin{table}[ht]
\small
\caption{Notations and explanations.}
% title of Table
\centering 
\begin{tabular}{c c}
\hline                      
Notations & Explanations  \\ [0.5ex]
\hline
$u, v$ & user and POI  \\
$r_{t}, r_{l}$ & temporal relation, spatial relation  \\
$r_{tl}$ &  spatio-temporal relation  \\
$r_{tlc}$ &  spatio-temporal and category-based relation  \\
$\mathcal{U}$ & user set   \\
$\mathcal{V}$ & POI set   \\
$\mathcal{C}$ & category context set   \\
$\tau, t$ & a timestamp and a time slot  \\
$g(\cdot)$ & embedding function  \\ 
$\mathcal{D}$ & a collection of all the triple sets \\
$\mathbb{R} ^d, \mathbb{R} ^k$ & $d$ and $k$ dimensional latent space \\
$\textbf{r}$ & relational embedding set \\
%$\textbf{r}_{tl}$ & relation embedding set with spatial-temporal effects \\
${\boldsymbol{M}}_r$ & project matrix set of relation $r$ \\
$S$ & positive triple set  \\
$S'$ & negative triple set \\
$\boldsymbol{e}^r_u$ & user representation of relation path $r$ \\
$\boldsymbol{e}^r_v$ & POI representation of relation path $r$ \\
$\boldsymbol{\phi}_u$ & user embedding set \\
$\boldsymbol{\phi}_v$ & POI embedding set \\
$\theta_d$ & distance threshold $\theta_d$ \\
\hline
\end{tabular}
\label{tb:notations}
\end{table}

\vspace{0.1cm}
\noindent{\textit{Problem 1.}}  \textbf{(\textit{Personalized POI recommendation})} Given an LBSN user check-in dataset and a query $q = (u, l, t, c)$, our target is to recommend each user with a personalized top-\textit{k} POIs they would be interested in visiting. We choose user $u$ from a user set $\mathcal{U}$, location $l\in\mathcal{L}$, time $t\in\mathcal{T}$ and POI category $c\in\mathcal{C}$.  %The query returns a top-k list of $v \in \mathcal{V}$. 

\vspace{0.1cm}
\noindent{\textit{Definition 1.}} \textbf{(\textit{User-POI})} A POI is a specific point location that user is interested in (for example a c\`afe or a restaurant). In our model, a POI has two attributes: identifier and category. We use $v\in\mathcal{V}$ to represent a POI identifier, where $\mathcal{V}$ is the POI identifier set. Category $c \in \mathcal{C}$ may  represent textual semantic information associated with a location.

\vspace{0.1cm}
\noindent{\textit{Definition 2.}} \textbf{(\textit{User check-in activity})}
A user check-in activity is made up of a quintuple, abbreviated as 5-tuple $(u, v, l, \tau, c)$ that represents user $u\in \mathcal{U}$ visiting POI $v\in \mathcal{V}$ at location $l\in \mathcal{L}$ and timestamp $\tau$. %\in\mathcal{T}$,
%where $\mathcal{T}=\{0,\cdots,23\}$ represents time quantized into 1h intervals.
To fit the timestamp into our proposed graph, we first map timestamp $\tau$ into the corresponding time slot $t$. A time slot $t$ splits a day into multiple equal time intervals based on hour(s).  

\vspace{0.1cm}
\noindent{\textit{Definition 3.}} \textbf{(\textit{User-POI based graph})} We define a user-POI graph $G$ by a collection of triples $(u, r, v)\in\mathcal{D}$%\equiv\mathcal{U}\times\mathcal{R}\times\mathcal{V}$
, in which $u, r,$ and $v$ denote the \textit{user}, \textit{relation} and \textit{POI}, and each user and a POI are connected by a specific relation. When we refer to vector embeddings corresponding to some $u$, $v$ and $r$, for brevity we write in bold $\mathbf{u},\, \mathbf{v} \in \mathbb{R}^k$ and  $\mathbf{r}\in \mathbb{R}^d$. We note that the dimensions of entity embeddings $\mathbf{u},\, \mathbf{v}$ and relational embeddings $\mathbf{r}$ may be different \ie, $k\neq d$.



\section{Preliminaries}
Below we explain the concepts and models that relate to this study. %First, we present knowledge graph embedding and then follow with a matrix factorization model.

%\subsection{knowledge graph embedding}
The role of a knowledge graph embedding is to embed components of a KG, including entities and relations, into a vector space \cite{wang2017knowledge}. A typical KG has a collection of triples $(h, r, t)$ and consists of millions of entities (nodes) and relations (different types of edges), in which $h, r,$ and $t$ denote the \textit{head entity}, \textit{relation} and \textit{tail entity} of a triple for which the head and tail entries are connected by some relation. Once pairs (\textit{head},\,\textit{relation}) and (\textit{tail},\,\textit{relation}) are embedded into some common latent vector space, their similarity (or relatedness) can be easily computed \ie, by  the dot-product.

The KG embedding can be performed in three simple steps:  (i) represent entities and relations in a vector space; (ii) define a score function for each triple to measure distance; %based on its calculated score;
and (iii) learn the entities and relational representations in the low-dimensional vector space.

Below, we summarize a state-of-art translational distance model called TransR \cite{lin2015learning}, a popular embedding for heterogeneous networks. Different from other translational distance-based models that assume entities and relations to lie within the same space, TransR  models entities and relations in distinct spaces. For each relation $r$, it sets a project matrix $\textbf{M}_r$ to project entities from the entity space to the relational space, that is head and tail embeddings become $\textbf{h}_r = \textbf{h} \textbf{{$\boldsymbol{M}$}}_r$ and
$\textbf{t}_r = \textbf{t} \textbf{{$\boldsymbol{M}$}}_r$, where $||\mathbf{h}_r + \mathbf{r} - \mathbf{t}_r||_2$
is a score function/distance.% is defined as the distance between $\textbf{h}_r + \textbf{r}$ and $\textbf{t}_r$.
%\begin{equation}
%f_r(h, t) = \parallel \textbf{h}_r + \textbf{r} - \textbf{t}_r \parallel ^2_2
%\end{equation}



% \paragraph{TransE} TransE \cite{bordes2013translating} is one of most representative translational distance model, which represents both entities and relations vectors in the same space. Given a triple ($h, r, t$), the embedded entities \textbf{h} and \textbf{t} are connected by a translation vector \textbf{r}, i.e., \textbf{h} + \textbf{r} $\approx$ \textbf{t} when ($h, r, t$) holds. The score function is defined as the following
% \begin{equation}
% f_r(h, t) = \parallel \textbf{h} + \textbf{r} - \textbf{t} \parallel ^2_2
% \end{equation}
% is low if ($h, r, t$) holds, and high otherwise. TransE has advantage for 1-to-1 relations and disadvantage for 1-to-N, N-to-1, and N-to-N relations.

% \paragraph{TransH} TransH \cite{wang2014knowledge} solves the 1-to-1 issue by introducing relation-specific hyperplanes. It models entities as vector, but each relation $r$ as a vector on a hyperplane with $\textbf{w}_r$. TransH assumes score function
% \begin{equation}
% f_r(h, t) = \parallel \textbf{h}_{\bot} + \textbf{r} - \textbf{t}_{\bot} \parallel ^2_2
% \end{equation}
% If restricting $\parallel \textbf{w}_r \parallel_2 = 1$, we can have $\textbf{h}_\bot = \textbf{h} - \textbf{w}_r^{\top} \textbf{h} \textbf{w}_r$ and $\textbf{t}_{\bot} = \textbf{t} - \textbf{w}_r^{\top} \textbf{t} \textbf{w}_r$. Entities can be associated with different relations by projecting entity embeddings into relation hyperplanes.

% \paragraph{TransR} Different from TransE and TransH that assume entities and relations within the same space, TransR \cite{lin2015learning} models entities and relations in distinct space. The score function is again defined as
% \begin{equation}
% f_r(h, t) = \parallel \textbf{h}_r + \textbf{r} - \textbf{t}_r \parallel ^2_2
% \end{equation}
% For each relation $r$, it sets a project matrix $\textbf{M}_r$, where $\textbf{h}_r = \textbf{h} \textbf{{\mathrm{M}}}_r$ and
% $\textbf{t}_r = \textbf{t} \textbf{{\mathrm{M}}}_r$.


% \subsection{Matrix factorization}
% Matrix factorization is a state-of-the-art approach in recommendation systems \cite{chen2018matrix}. Given the observed entries in a $|U| \times |V|$ user-item rating matrix $F$, the goal of MF is to find a low-rank matrix for users $U \in \mathbb{R}^{K \times |U|}$ and items $V \in \mathbb{R}^{K \times |V|}$ such that $F \approx U^{\top} V$. The probability of a user $u$ like an item $v$ is defined as 
% \begin{equation}
%   P(F_{uv}) \propto U^{\top}_u V_v 
% \end{equation}
% The corresponding objective function computes the mapping user and item factor matrices by fitting the observed ratings in the training set.

% \begin{equation}\label{eq:mf_train_func}
% \underset{U, V}{min} \sum_{(u,v)\in \Omega} (P_{uv} -  U_u^{\top} V_v )^2 + \lambda (\parallel U \parallel^2_F + \parallel V \parallel^2_F),
% \end{equation}
% where $(u,v)\in \Omega$ demonstrate the rating of user $u$ for item $v$ is observed. $\parallel \cdot \parallel^2_F$ denotes the Frobenius norm.

